Wasserstein Least Squares: A Canonical Regression Method for Probability Distributions

We perform a mathematical and statistical analysis of the Wasserstein least squares problem, a regression method for vector-valued covariates and distribution-valued responses. Our proposal contrasts with other distributional regression methods by having a direct interpretation in terms of random variables, as a nonparametric analogue of the classic random-effects model. On the mathematical side, we use a strategy of Lavenant (2024) to show that Wasserstein least squares is the canonical extension of Euclidean least squares to the space of probability distributions from the perspective of convex analysis; this viewpoint gives rise to multimarginal and dual formulations of the Wasserstein least squares problem, extending a similar theory for Wasserstein barycenters. We perform a statistical analysis of the Wasserstein least squares problem under the template deformation model, showing, surprisingly, that estimation is possible at the n^{-1/2} rate. As a special case, we obtain improved rates of estimation for Wasserstein barycenters, which are an exponential improvement over those established by Ahidar-Coutrix, Le Gouic and Paris (2020). Finally, we propose a heuristic particle method for Wasserstein least squares and use it to conduct a novel analysis of large-scale demographic data from the RAND Health and Retirement Study.

==> commands.tex <==
\usepackage{amsmath, amssymb, color,mathtools}
\usepackage{amsthm}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{xcolor,colortbl}
\RequirePackage{hypernat}
\usepackage[capitalize]{cleveref}
\usepackage{comment}
\usepackage{color}
\usepackage{amsfonts, fancybox}
\usepackage{amssymb}
\usepackage[american]{babel}
\usepackage{color}
\usepackage{dcolumn}
\usepackage[format=hang, justification=justified, singlelinecheck=false]{subcaption}
\usepackage{flafter, bm, dsfont}
\usepackage[section]{placeins}

\usepackage{multirow}
\usepackage{color}
\usepackage{amsmath}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{amssymb}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{wrapfig}

\usepackage{amssymb, latexsym}

\usepackage{graphicx}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}

\usepackage{color}
\usepackage{algorithm}
\usepackage{algpseudocode}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{exe}{Exercise}
\newtheorem{exa}{Example}
\newtheorem{fact}{Fact}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{conj}{Conjecture}
\newtheorem{remark}{Remark}
\newtheorem{assume}{Assumption}
\newtheorem{discussion}{Discussion}
\newtheorem{conc}{Conclusion}

\crefname{condition}{condition}{conditions}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\pp}{p}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\p}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}

\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\PP}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\DS}{\displaystyle}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator\supp{supp}
\DeclareMathOperator\Span{span}
\DeclareMathOperator\vect{vec}
\DeclareMathOperator{\Id}{Id}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\eps}{\varepsilon}
\newcommand{\del}{\delta}
\newcommand{\re}{\R}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\plusminus}{\raisebox{.2ex}{$\scriptstyle\pm$}}
\newcommand{\nnz}{\text{nnz}}
\newcommand{\KL}{\cK}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\diag}{\mathbf{D}}
\newcommand{\ones}{\bone_n}
\newcommand{\tildo}{\widetilde{O}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\bone}{\mathbf{1}}

\newcommand{\errr}{\text{err}_r}
\newcommand{\errrp}{\text{err}_r^{(+)}}
\newcommand{\errrn}{\text{err}_r^{(-)}}
\newcommand{\errc}{\text{err}_c}
\newcommand{\errcp}{\text{err}_c^{(+)}}
\newcommand{\errcn}{\text{err}_c^{(-)}}
\newcommand{\Cinfty}{\|C\|_{\infty}}

\newcommand{\zeroesr}{\text{zeroes}_r}
\newcommand{\zeroesc}{\text{zeroes}_c}

\newcommand{\Pavg}{P_{\text{avg}}}
\newcommand{\Pavgex}{P_{\text{avg}}^{\text{exact}}}
\newcommand{\Ptex}{P_t^{\text{exact}}}
\newcommand{\Pbar}{{\bar{P}}}
\newcommand{\Pprime}{P'}
\newcommand{\Pex}{Q^{\text{sink}}}
\newcommand{\Qsink}{\Pex}
\newcommand{\Poptprime}{(P^*)'}

\newcommand{\U}{\cU_{r,c}}
\newcommand{\Ubar}{\cU_{\rbar, \cbar}}
\newcommand{\Uprime}{\cU_{r', c'}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\Peta}{P_\eta}
\newcommand{\sink}{\Pi_{\cS}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\be}{\boldsymbol{e}}

\newcommand{\WGrad}{\nabla\!\!\!\!\nabla}

\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}
\DeclareMathOperator{\law}{Law}

\newcommand{\EEuc}{E}
\newcommand{\EWas}{\cE}
\newcommand{\dd}{\, \mathrm{d}}
